Communication Efficient Distributed Learning for Kernelized Contextual Bandits

We tackle the communication efficiency challenge of learning kernelized contextual bandits in a distributed setting. Despite the recent advances in communication-efficient distributed bandit learning, existing solutions are restricted to simple models like multi-armed bandits and linear bandits, which hamper their practical utility. In this paper, instead of assuming the existence of a linear reward mapping from the features to the expected rewards, we consider non-linear reward mappings, by letting agents collaboratively search in a reproducing kernel Hilbert space (RKHS). This introduces significant challenges in communication efficiency as distributed kernel learning requires the transfer of raw data, leading to a communication cost that grows linearly w.r.t. time horizon $T$. We addresses this issue by equipping all agents to communicate via a common Nystr\"{o}m embedding that gets updated adaptively as more data points are collected. We rigorously proved that our algorithm can attain sub-linear rate in both regret and communication cost.

==> Arxiv/exp.tex <==
\section{Experiments}
In order to evaluate \algtwo{}'s effectiveness in reducing communication cost, we performed extensive empirical evaluations on both synthetic and real-world datasets, and the results (averaged over 3 runs) are reported in Figure \ref{fig:synthetic_exp_results}, \ref{fig:uci_exp_results} and \ref{fig:recommendation_exp_results}, respectively.
We included \algone{}, 
% a distributed version of BBKB \citep{calandriello2020near} adapted to our problem (named as DisBKB), 
DisLinUCB \citep{wang2019distributed}, OneKernelUCB, and NKernelUCB \citep{chowdhury2017kernelized} as baselines, where One-KernelUCB learns a shared bandit model across all clients' aggregated data where data aggregation happens immediately after each new data point becomes available, and N-KernelUCB learns a separated bandit model for each client with no communication. For all the kernelized algorithms, we used the Gaussian kernel $k(x, y) = \exp(-\gamma \lVert x-y \rVert^{2})$.
We did a grid search of $\gamma \in \{0.1, 1, 4\}$ for kernelized algorithms, and set $D=20$ for DisLinUCB and \algone{}, $D=5$ for \algtwo{}. For all algorithms, instead of using their theoretically derived exploration coefficient $\alpha$, we followed the convention \cite{li2010contextual,zhou2020neural} to use grid search for $\alpha$ in $\{0.1, 1, 4\}$.

\begin{figure}[t]
% \vspace{-2mm}
\centering 
\subfigure[$f_{1}(\bx)=\cos(3 \bx^{\top} \btheta_{\star})$]{\label{fig:a}\includegraphics[width=0.48\textwidth]{imgs/regret_comm_cosine_avg_nobkb.png}}
\subfigure[$f_{2}(\bx)=(\bx^{\top} \btheta_{\star})^{3} - 3(\bx^{\top} \btheta_{\star})^{2} - (\bx^{\top} \btheta_{\star}) + 3$]{\label{fig:b}\includegraphics[width=0.48\textwidth]{imgs/regret_comm_cubic_avg_nobkb.png}}
% \subfigure[Mushroom]{\label{fig:c}\includegraphics[width=0.32\textwidth]{NeurIPS2022/imgs/regretVScommCost_plot_11_19_16_08T2000N20datasetMushroom.pdf}}
\caption{Experiment results on synthetic datasets.}
\label{fig:synthetic_exp_results}
% \vspace{-2mm}
\end{figure}


\paragraph{Synthetic dataset}
We simulated the distributed bandit setting defined in Section \ref{subsec:problem_formulation}, with $d=20,T=100, N=100$ ($NT=10^{4}$ interactions in total). In each round $l \in [T]$, each client $i \in [N]$ (denote $t=N(l-1)+i$) selects an arm from candidate set $\cA_{t}$, 
where $\cA_{t}$ is uniformly sampled from a $\ell_2$ unit ball, with $|\cA_{t}|=20$.
% where $\cA_{t}$ is uniformly sampled from a $\ell_2$ unit sphere,
% Following \citep{zhou2020neural}, 
% The reward function $f(\cdot)$ is one of the following
Then the corresponding reward is generated using one of the following reward functions:
% and arm set $\cA$ 
% are simulated:
\begin{align*}
% & f_{1}(\bx) = 10( \bx^{\top} \btheta_{\star})^{2}  \\
& f_{1}(\bx) = \cos(3 \bx^{\top} \btheta_{\star}) \\
& f_{2}(\bx) = (\bx^{\top} \btheta_{\star})^{3} - 3(\bx^{\top} \btheta_{\star})^{2} - (\bx^{\top} \btheta_{\star}) + 3
% & f(\bx) = \cos(3 \bx^{\top} \btheta), \text{and $\cA$ uniformly sampled from a $\ell_2$ unit ball with $|\cA|=200$}  \\
% & f(\bx) = \exp(- (\bx^{\top} \btheta - 1)^{2}), \text{and $\cA$ uniformly sampled from $[0,1]^{d}$ with $|\cA|=200$}
%   f(\bx) =
%     \begin{cases}
%       & 10( \bx^{\top} \btheta)^{2}, \text{with $\btheta$ uniformly sampled from a $\ell_2$ unit ball}, \\
%     %   & \bx^{\top} \Theta^{\top}\Theta \bx, \text{with each entry of $\Theta \in \bR^{d \times d}$ an iid sample from $\cN(0,1)$ }, \\
%       & \cos(3 \bx^{\top} \btheta), \text{with $\btheta$ uniformly sampled from a $\ell_2$ unit ball}.
%     \end{cases}       
\end{align*}
where the parameter $\btheta_{\star}$ is uniformly sampled from a $\ell_2$ unit ball.


% For the experiments on synthetic dataset, we simulated the environment in Section \ref{subsec:problem_formulation}.

% The number of rounds T = 10 000. The contextual vectors {x1,1, . . . , xT ,K} are chosen uniformly at random from the
% unit ball. The reward function h is one of the following: where each entry of A ∈ R
% d×d
% is randomly generated from
% N(0, 1), a is randomly generated from uniform distribution
% over unit ball. For each hi(·), the reward is generated by
% rt,a = hi(xt,a) + ξt, where ξt ∼ N(0, 1).
\paragraph{UCI Datasets}
To evaluate \algtwo{}'s performance in a more challenging and practical scenario, we performed experiments using real-world datasets: MagicTelescope, Mushroom and Shuttle from the UCI Machine Learning Repository \citep{Dua:2019}. To convert them to contextual bandit problems, we pre-processed these datasets following the steps in \citep{filippi2010parametric}. In particular, we partitioned the dataset in to $20$ clusters using k-means, and used the centroid of each cluster as the context vector for the arm and the averaged response variable as mean reward (the response variable is binarized by
associating one class as $1$, and all the others as $0$). Then we simulated the distributed bandit learning problem in Section \ref{subsec:problem_formulation} with $|\cA_{t}|=20$, $T=100$ and $N=100$ ($NT=10^{4}$ interactions in total).

\begin{figure}[t]
% \vspace{-2mm}
\centering 
\subfigure[MagicTelescope]{\label{fig:c}\includegraphics[width=0.32\textwidth]{imgs/regret_comm_magictelescope_avg_nobkb.png}}
\subfigure[Mushroom]{\label{fig:d}\includegraphics[width=0.32\textwidth]{imgs/regret_comm_mushroom_avg_nobkb.png}}
\subfigure[Shuttle]{\label{fig:e}\includegraphics[width=0.32\textwidth]{imgs/regret_comm_shuttle_avg_nobkb.png}}
\caption{Experiment results on UCI datasets.}
\label{fig:uci_exp_results}
% \vspace{-2mm}
\end{figure}

\begin{figure}[t]
% \vspace{-2mm}
\centering 
\subfigure[MovieLens]{\label{fig:f}\includegraphics[width=0.48\textwidth]{imgs/regret_comm_movielens_avg_nobkb.png}}
\subfigure[Yelp]{\label{fig:g}\includegraphics[width=0.48\textwidth]{imgs/regret_comm_yelp_avg_nobkb.png}}
\caption{Experiment results on MovieLens \& Yelp datasets.}
\label{fig:recommendation_exp_results}
% \vspace{-2mm}
\end{figure}

\paragraph{MovieLens and Yelp dataset}
Yelp dataset, which is released by the Yelp dataset challenge, consists of 4.7 million rating entries for 157 thousand restaurants by 1.18 million users. MovieLens is a dataset consisting of 25 million ratings between 160 thousand users and 60 thousand movies \citep{harper2015movielens}. Following the pre-processing steps in \citep{ban2021ee}, we built the rating matrix by choosing the top 2000 users and top 10000 restaurants/movies and used singular-value decomposition (SVD) to extract a 10-dimension feature vector for each user and restaurant/movie. We treated rating greater than $2$ as positive. 
We simulated the distributed bandit learning problem in Section \ref{subsec:problem_formulation} with $T=100$ and $N=100$ ($NT=10^{4}$ interactions in total).
In each time step, the candidate set $\cA_{t}$ (with $|\cA_{t}|=20$) is constructed by sampling an arm with reward $1$ and nineteen arms with reward $0$ from the arm pool, and the concatenation of user and restaurant/movie feature vector is used as the context vector for the arm (thus $d=20$).


\paragraph{Discussions}
When examining the experiment results presented in Figure \ref{fig:synthetic_exp_results}, \ref{fig:uci_exp_results} and \ref{fig:recommendation_exp_results}, we can first look at the cumulative regret and communication cost of OneKernelUCB and NKernelUCB, which correspond to the two extreme cases where the clients communicate in every time step to learn a shared model, and each client learns its own model independently with no communication, respectively.
OneKernelUCB achieves the smallest cumulative regret in all experiments, while also incurring the highest communication cost, i.e., $O(T N^{2} d)$. This demonstrates the need of efficient data aggregation across clients for reducing regret. 

Second, we can observe that \algone{} incurs the second highest communication cost in all experiments due to the transfer of raw data, as we have discussed in Remark \ref{rmk:1}, which makes it prohibitively expensive for distributed setting.
On the other extreme, we can see that DisLinUCB incurs very small communication cost thanks to its closed-form solution, but fails to capture the complicated reward mappings in most of these datasets, e.g. in Figure \ref{fig:a}, \ref{fig:d} and \ref{fig:f}, it leads to even worse regret than NKernelUCB that learns a kernelized bandit model independently for each client.
% , despite being equipped with an event-trigger, the transfer of raw data points.

In comparison, the proposed \algtwo{} algorithm enjoys the best of both worlds in most cases, i.e., it can take advantage of the superior modeling power of kernels to reduce regret, while only requiring a relatively low communication cost for clients to collaborate. On all the datasets, \algtwo{} achieved comparable regret with \algone{} that maintains exact kernelized estimators, and sometimes even getting very close to OneKernelUCB, e.g., in Figure \ref{fig:b} and \ref{fig:c}, but its communication cost is only slightly higher than that of DisLinUCB.

==> Arxiv/intro.tex <==
\section{Introduction} \label{sec:intro}
% As a classic model for sequential decision making problems, 
Contextual bandit algorithms have been widely used for a variety of real-world applications, including recommender systems \citep{li2010contextual}, display advertisement \citep{li2010exploitation} and clinical trials \citep{durand2018contextual}. While most existing bandit solutions assume a centralized setting (i.e., all the data reside in and all the actions are taken by a central server), 
%motivated by the increasing amount of large scale distributed applications, 
there is 
%a growing demand to keep data decentralized and push the learning of bandit models to the client side. This has led to the 
increasing research effort on distributed bandit learning lately \citep{wang2019distributed,dubey2020differentially,shi2021federated,huang2021federated,li2022asynchronous},
where $N$ clients, under the coordination of a central server, collaborate 
% with limited communication bandwidth 
to minimize the overall cumulative regret incurred over a finite time horizon $T$. In many distributed application scenarios, communication is the main bottleneck, e.g., communication in a network of mobile devices can be slower than local computation by several orders of magnitude \citep{huang2013depth}.
Therefore, it is vital for distributed bandit learning algorithms to attain sub-linear rate (w.r.t. time horizon $T$) in both cumulative regret and communication cost.

However, prior works in this line of research are restricted to linear models \citep{wang2019distributed}, which could oversimplify the problem and thus leads to inferior performance in practice. In centralized setting, kernelized bandit algorithms, e.g., KernelUCB \citep{valko2013finite} and IGP-UCB \citep{chowdhury2017kernelized}, are proposed to address this issue by modeling the unknown reward mapping as a non-parametric function lying in a reproducing kernel Hilbert space (RKHS), i.e., the expected reward is linear w.r.t. an action feature map of possibly infinite dimensions.
Despite the strong modeling capability of kernel method, collaborative exploration in the RKHS gives rise to additional challenges in designing a communication efficient bandit algorithm.
Specifically, unlike distributed linear bandit where the clients can simply communicate the $d \times d$ sufficient statistics \citep{wang2019distributed}, where $d$ is the dimension of the input feature vector, the \emph{joint kernelized estimation} of the unknown reward function requires communicating either 1) the $p \times p$ sufficient statistics in the RKHS, where $p$ is the dimension of the RKHS that is possibly infinite, or 2) the set of input feature vectors that grows linearly w.r.t. $T$. Neither of them is practical due to the huge communication cost. 
% Neither of them is communication-efficient.
% \huazheng{A table of regret and communication order}

In this paper, we propose the first communication efficient algorithm for distributed kernel bandits, which tackles the aforementioned challenge via a low-rank approximation of the empirical kernel matrix. 
% Nystr\"{o}m method
% Kernel matrix approximation is commonly used in supervised learning for reducing the computation cost.
In particular, we extended the Nystr\"{o}m method \citep{nystrom1930praktische} to distributed learning for kernelized contextual bandits. In this solution, all clients first project their local data to a finite RKHS spanned by a common dictionary, i.e., a small subset of the original dataset, and then they only need to communicate the embedded statistics for collaborative exploration. To ensure effective regret reduction after each communication round, as well as ensuring the dictionary remains representative for the entire distributed dataset throughout the learning process, the frequency of dictionary update and synchronization of embedded statistics is controlled by measuring the amount of new information each client has gained since last communication.
We rigorously prove that the proposed algorithm incurs an $O(N^{2} \gamma_{NT}^{3})$ communication cost, where $\gamma_{NT}$ is the maximum information gain that is known to be $O\bigl(\log (NT) \bigr)$ for kernels with exponentially decaying eigenvalues, which includes the most commonly used Gaussian kernel, while attaining the optimal $O(\sqrt{NT}\gamma_{NT})$ cumulative regret.
% without sacrificing the cumulative regret. 
% \huazheng{Need explicit regret and communication order.} 
% Extensive empirical evaluations also validate the effectiveness of our algorithm.
